SUGAR: Efficient Subgraph-level Training via Resource-aware Graph Partitioning

Graph Neural Networks (GNNs) have demonstrated a great potential in a variety of graph-based applications, such as recommender systems, drug discovery, and object recognition. Nevertheless, resource-efficient GNN learning is a rarely explored topic despite its many benefits for edge computing and Internet of Things (IoT) applications. To improve this state of affairs, this work proposes efficient subgraph-level training via resource-aware graph partitioning (SUGAR). SUGAR first partitions the initial graph into a set of disjoint subgraphs and then performs local training at the subgraph-level. We provide a theoretical analysis and conduct extensive experiments on five graph benchmarks to verify its efficacy in practice. Our results show that SUGAR can achieve up to 33 times runtime speedup and 3.8 times memory reduction on large-scale graphs. We believe SUGAR opens a new research direction towards developing GNN methods that are resource-efficient, hence suitable for IoT deployment.

==> 3.method.tex <==
\section{Our Proposed Method}
\subsection{Problem Formulation} \label{sec.form}
Given a graph $\mathcal{G} = (\mathcal V,\mathcal E)$, where $\mathcal V$ is the node set and $\mathcal E$ represents the set of edges. Let $N=|\mathcal V|$ denote the number of nodes and $A \in R^{N\times N}$ be the adjacency matrix of $\mathcal{G}$. Every node $i$ is characterized by a $F$-dimensional feature vector $x_i \in R^{1 \times F}$. We use $X \in R^{N \times F}$ to represent the feature matrix of all nodes in $\mathcal G$. 
% $A_{ij} = 1 $ if there is an edge between node $i$ and $j$ and 0 otherwise.

Consider a general node-level prediction problem, \eg, node classification or node regression. Suppose we have a neural network $f(\cdot)$ parameterized by $W$ that predicts the label for each node given its features, the general objective is to minimize the following loss function with respect to model weights $W$:
\begin{equation}
	\min_W \frac{1}{N}\sum_{i=1}^N \mathcal L(f(x_i; W), y_i)
	\label{eq.centralized}
\end{equation}

where $\mathcal L$ denotes the cross entropy for a classification problem and the regression loss for node regression tasks, respectively. Without loss of generality, we consider the node classification problem throughout this paper. Variables $y_i$ represent the ground truth label for node $i$. 

% Note that $f(\cdot)$ represents a general classifier, for instance, a simple MLP where $f(x_i) = \sigma(Wx_i + b)$.

Suppose there are $K$ devices available for training, and let $\mathcal B_{MEM}^i$ denote the memory budget of device $i$. Motivated by the notorious inefficiency that centralized graph learning suffers from, we aim at \emph{distributing the training process} to improve the training scalability. The key is to assign all $N$ nodes of graph $\mathcal G$ to $K$ devices, and maintain a local model on \emph{each} device, \ie, model $f(W_i)$ for device $i$. This becomes a graph partitioning problem, as formulated below.
 
A partitioning strategy $\mathcal{P}: \mathcal V \rightarrow (\mathcal V_1, \mathcal V_2, \cdots, \mathcal V_K)$ divides the node set $\mathcal V$ into $K$ subsets such that 
\begin{equation}
	\begin{split}
	 	\cup_i \mathcal V_i & = \mathcal V, \\
	 \ H(\mathcal{SG}_i,W_i)  < & \mathcal B_{MEM}^i,  \forall i \in \{1, 2, \cdots, K\}
	\end{split}
	\label{eq.constraint}
\end{equation}
where $\mathcal{SG}_i$ denotes the subgraph induced by node set $\mathcal V_i$. $H$ is a static function that maps a given subgraph $\mathcal{SG}_i$ and the corresponding model $W_i$ to the memory requirements for training. For maximum generality, here we do not require $\mathcal V_i \cap \mathcal V_j = \varnothing$; in other words, a node $i$ can be assigned to more than one hardware device. 

%We find that this kind of redundancy leads to better accuracy in the experiments.

As opposed to the centralized setting, in our formulation, there are $K$ distinct (local) models $\mathbf{W}=\{W_i\}_{i=1}^K$ instead of a single (global) model. A node can exist in multiple hardware devices, and let $\mathcal P_i$ be the set of devices where node $i$ is assigned to. $\mathbf{W}_i=\{W_k\}_{k\in \mathcal P_i}$ represents the set of local models corresponding to $\mathcal P_i$. We average the outputs from local models in $\mathbf{W}_i$ as the final prediction for node $i$. Consequently, we rewrite the loss function in Equation \ref{eq.centralized} as:
\begin{equation}
	\begin{split}
 \min_{\mathcal P, \mathbf{W}} \ \ & \frac{1}{N}\sum_{i=1}^N \mathcal L(f(x_i; \mathbf{W}_i), y_i) \text{ \ where} \\
 \ & f(x_i;\mathbf{W}_i)  = \frac{1}{|\mathcal P_i|} \sum_{k \in \mathcal P_i} f(x_i;W_k) \\
\text{subject to: \ } & \mathcal{P}:\mathcal V \rightarrow (\mathcal V_1, \mathcal V_2, \cdots, \mathcal V_K), \ \cup_i \mathcal V_i = \mathcal V,\\
H(&\mathcal{SG}_i,W_i)  < \mathcal B_{MEM}^i, \forall i \in \{1, 2, \cdots, K\} \\
\end{split}
\label{eq.formulation}
\end{equation}
where $\mathcal{P}$ is the partitioning strategy defined above and $\mathbf{W}$ is the set of all $K$ local models. The above formulation incurs two critical \emph{subproblems}: (1) How to train $K$ local models with minimum possible communication among devices? (2) How to find an optimal partitioning strategy $\mathcal P$ subject to resource constraints? We answer these questions in the following sections.

\subsection{Subgraph-level GNN Training}
This section discusses the problem of \emph{training-time communication}. In the current formulation, if $|\mathcal P_i| > 1$, \ie, a node $i$ is assigned to multiple devices, calculating its loss and back-propagation will involve heavy communication among multiple models in $\mathbf{W}_i$. To address this problem and reduce the training-time communication to zero, we provide the following result.

% The objective function in Equation \ref{eq.formulation} can be written as:
% \begin{equation}
% 	\frac{1}{N} \sum_{i=1}^N \mathcal L(\frac{1}{|\mathcal P_i|} \sum_{k\in \mathcal P_i}f(x_i;W_k), y_i)
% 	\label{eq.objective}
% \end{equation}  

% Given that cross entropy loss $\mathcal L(f, y)$ is convex with respect to $f$, we have $\mathcal L(\frac{1}{|\mathcal P_i|} \sum_{k\in \mathcal P_i}f(x_i;W_k), y_i) \leq \frac{1}{|\mathcal P_i|} \sum_{k\in \mathcal P_i}\mathcal L(f(x_i;W_k), y_i)$ using Jensen's inequality. Therefore, the upper bound of Equation \ref{eq.objective} is:
% $
%     \frac{1}{N} \sum_{i=1}^N \frac{1}{|\mathcal P_i|} \sum_{k\in \mathcal P_i}\mathcal L(f(x_i;W_k), y_i)
% 	\label{eq.node-level}
% $.

% This is equivalent to Equation \ref{eq.ub-objective} below by changing the operation order and regrouping the indices:
% \begin{equation}
%     \begin{aligned}
% 	& \frac{1}{K} \sum_{k=1}^K \frac{1}{|\mathcal V_k|} \sum_{i\in \mathcal V_k} \frac{|\mathcal V_k|}{|\mathcal P_i|}\mathcal L(f(x_i;W_k), y_i)  \\
% 	= &\frac{1}{K} \sum_{k=1}^K  \sum_{i\in \mathcal V_k} \frac{1}{|\mathcal P_i|}\mathcal L(f(x_i;W_k), y_i)  
% 	\end{aligned}
% 	\label{eq.ub-objective}
% \end{equation}  

% Now, we switch the perspective from `node-level' (\ie, minimizing the loss for each node) to `device-level' (\ie, minimizing the loss per device) and show that optimizing the latter reduces the upper bound of the original objective in Equation \ref{eq.objective}. Thus, our new training objective can be described as:
% \begin{equation}
% 	\begin{split}
% \min_{\mathcal P, \mathbf W} \   F(\mathcal P, \mathbf{W}) \triangleq \frac{1}{K}\sum_{k=1}^KF_k(\mathcal{SG}_k; W_k) \\
% 	  F_k(\mathcal{SG}_k; W_k)= \sum_{i\in \mathcal V_k}\frac{1}{|\mathcal P_i|} \mathcal L(f(x_i;W_k), y_i) 
% \end{split}
% \label{eq.new-formulation}
% \end{equation}

% where $\mathcal V_k$ is the node set of subgraph $\mathcal{SG}_k$. We define $F$ to be a global objective function and $F_k$ to be the local objective function for device $k$. As it can be seen in Equation \ref{eq.new-formulation}, the training-time communication among devices is no longer required in the new formulation, hence training happens only at subgraph-level.

\begin{prop}
The upper bound of the objective function in Equation \ref{eq.formulation} is given below.
\begin{equation}
\text{Loss} \leq \frac{1}{K} \sum_{k=1}^K  \sum_{i\in \mathcal V_k} \frac{1}{|\mathcal P_i|}\mathcal L(f(x_i;W_k), y_i) 
\end{equation}
\label{prop.ub}
\end{prop}
% \vspace{-2mm}
\textit{Proof.} Given that cross entropy loss $\mathcal L(f, y)$ is convex with respect to $f$, we have $\mathcal L(\frac{1}{|\mathcal P_i|} \sum_{k\in \mathcal P_i}f(x_i;W_k), y_i) \leq \frac{1}{|\mathcal P_i|} \sum_{k\in \mathcal P_i}\mathcal L(f(x_i;W_k), y_i)$ using Jensen's inequality. By changing the operation order and regrouping the indices, we have $\frac{1}{N} \sum_{i=1}^N \frac{1}{|\mathcal P_i|} \sum_{k\in \mathcal P_i}\mathcal L(f(x_i;W_k), y_i) = & \frac{1}{K} \sum_{k=1}^K \sum_{i\in \mathcal V_k} \frac{1}{|\mathcal P_i|}\mathcal L(f(x_i;W_k), y_i)  $
% By changing the operation order and regrouping the indices, we show below that minimizing the loss per node is equivalent to minimizing the loss per hardware device:
% \begin{equation}
%     \begin{aligned}
%     & \frac{1}{N} \sum_{i=1}^N \frac{1}{|\mathcal P_i|} \sum_{k\in \mathcal P_i}\mathcal L(f(x_i;W_k), y_i)  \\
% 	 = & \frac{1}{K} \sum_{k=1}^K \frac{1}{|\mathcal V_k|} \sum_{i\in \mathcal V_k} \frac{|\mathcal V_k|}{|\mathcal P_i|}\mathcal L(f(x_i;W_k), y_i)  
% 	\end{aligned}
% 	\label{eq.ub-objective}
% \end{equation}  
Thus the proof is complete.

Proposition \ref{prop.ub} allows us to shift the perspective from `node-level' to `device-level'. Instead of directly optimizing the original objective in Equation \ref{eq.formulation}, we adopt its upper bound as our new training objective. Optimizing the new objective naturally reduces the upper bound of the original one and reduces model communication to zero. The new problem formulation can be described as:
% \begin{equation}
% 	\begin{split}
% \min_{\mathcal P, \mathbf W} \   F(\mathcal P, \mathbf{W}) \triangleq \frac{1}{K}\sum_{k=1}^KF_k(\mathcal{SG}_k; W_k) \\
% 	  F_k(\mathcal{SG}_k; W_k) \triangleq \sum_{i\in \mathcal V_k}\frac{1}{|\mathcal P_i|} \mathcal L(f(x_i;W_k), y_i) 
% \end{split}
% \label{eq.new-formulation}
% \end{equation}
\begin{equation}
	\begin{split}
 \min_{W_k} \  & F_k(\mathcal{SG}_k; W_k), \forall k \in \{1, 2, \cdots, K\} \\
	 F_k(\mathcal{SG}_k&; W_k) \triangleq \sum_{i\in \mathcal V_k}\frac{1}{|\mathcal P_i|} \mathcal L(f(x_i;W_k), y_i) 
\end{split}
\label{eq.new-formulation}
\end{equation}
We define $F_k$ to be the local objective function of device $k$. As can be seen in Equation \ref{eq.new-formulation}, the updates of local models are decoupled from each other, thus inter-device communication during training is no longer required.

To sum up, we propose subgraph-level local GNN training. As opposed to a centralized model, \emph{we train multiple local models} $\mathbf{W}=\{W_k\}_1^K$ in parallel. Each model $W_k$ takes a (different) subgraph $\mathcal{SG}_k$ as input for training. In the new formulation, communication among devices is reduced to zero. This can greatly speed up the training process.
% with $K$ available devices
% Of note, the updates of local models are decoupled from each other, thus requiring no inter-device communication during training.

\begin{figure*}[thp]
\centering
\includegraphics[width=0.9\textwidth]{figs/framework_new_v2.pdf} 
% \includegraphics[width=0.85\textwidth]{figs/draft.pdf} 
\caption{The proposed \sg consists of two stages: (a) graph partitioning and (b) subgraph-level GNN training. Graph partitioning involves three steps: (1) transform the input graph $\mathcal{G}$ to a weighted graph $\mathcal{G}^w$; (2) apply METIS to the weighted graph $\mathcal{G}^w$, where edges with large weights are more likely to be preserved; (3) (optional) expand the node set of the obtained subgraph according to memory budgets. While vanilla training is likely to run out of memory when the graph size is large and distributed GNN approaches require heavy intermediate communication, \sg provides a solution that is memory efficient and requires no inter-device communication.}
% In subgraph-level GNN training, we train a set of local GNN models in parallel, requiring no communication during training time. Significant speedup as well as memory efficiency are achieved at the subgraph-level.
\label{fig.framework}
\end{figure*}
% Given the input graph and available devices, \sg partitions the graph into a set of subgraphs, with each subgraph being placed on one device.

\subsection{Proposed Graph Partitioning Method}
In this section, we describe how to obtain the set of subgraphs $\{\mathcal{SG}_k\}_1^K$ from a given input graph $\mathcal{G}$.

Suppose $f(\cdot)$ is a $L$-layer GNN. To update a node $i$'s representation, the features of all neighbors of node $i$ are aggregated and then combined with node $i$'s representation through a non-linear function. Therefore, the exact GNN algorithm requires the original graph topology (\ie, adjacency matrix $A$), as well as node features as inputs.

\textbf{Approximation of $\mathbf{A}$}. In our formulation, we restrict the neighborhood search of a node $i$ within the subgraph $i$ belongs to. For the local GNN model $W_k$ associated with $k$-th device, we adopt the adjacency matrix of $\mathcal{SG}_k$, denoted by $A_{k}$, to approximate $A$. Taking $K$ subgraphs together into consideration, we provide the following matrix form:
\begin{equation}
	A = \tilde A + E 
	\label{eq.matrix_apx}  
\end{equation}

where $\tilde A = \begin{bmatrix}
		A_{1} & \cdots & 0 & \cdots & 0 \\
		\vdots & \ddots &  &  & \vdots \\
		0 & & A_{k} & & 0\\
		\vdots & & & \ddots & \vdots \\ 
		0 & \cdots & 0 & \cdots & A_{K}
	\end{bmatrix} = diag(A)$, and $E$ is the \emph{error matrix}, representing differences between $A$ and $\tilde A$.

We employ $\tilde A$ for training GNN models. This approximation of $A$ yields three benefits: (1) computational efficiency (2) low memory requirements (3) zero communication during training time. Next, we use a simple GCN to demonstrate these benefits. 

% \textbf{Complexity Analysis}.
\textbf{Complexity Analysis}. The $l$-th layer GCN model takes the form of:
\begin{equation}
	Z^{(l+1)} = f(X^{(l)},A;W^{(l)}) = \sigma(A^{norm}X^{(l)}W^{(l)})
\end{equation}
where $A^{norm}=\hat D^{-1/2}\hat A \hat D^{1/2}, \hat A = A + I_N, \hat D_{ii}=\sum_j\hat A_{ij}$ denotes the normalized version of $A$ ($I_N$ is an $N$-dimensional identity matrix). $X^{(l)}\in R^{N\times F_l}$ and $Z^{(l+1)}\in R^{N\times F_{l+1}}$ denotes the input and output node feature matrix for layer $l$, respectively. $W \in R^{F_l\times F_{l+1}}$ represent the $l$-th layer weights of the GCN. $F_l$ and $F_{l+1}$ represent the input and output feature numbers, respectively. Therefore, the \emph{training time complexity} is $\mathcal O(|\mathcal E|F_l + NF_l F_{l+1})$ and \emph{memory complexity} is $\mathcal O(NF_{l+1}+F_l F_{l+1})$. We make two observations here: (a) Real-world graphs are usually sparse and the average degree is generally smaller than feature number $F_{l+1}$. Thus the second term dominates in the time complexity; (b) For large-scale graphs, the number of nodes $N$ is much greater than the number of features. Consequently, $\mathcal O(NF_{l+1})$ dominates in the memory complexity. 

It is easy to verify that the number of nodes $N$ imposes a computation hurdle on GNN training. By partitioning the input graph into $K$ subgraphs, we reduce the number of nodes $N$ to $N_k=|\mathcal{V}_k|$ for every local model. Since $N_k $ is about $1/K$ of $N$, the proposed approach is expected to achieve up to $K$ times speedup, and as small as $1/K$ of the original memory requirements. Moreover, by substituting $A$ with $\tilde A$ in the propagation rule under the distributed setting discussed in the previous section, we have:
\begin{equation}
	Z^{(l+1)} = \sigma (\begin{bmatrix}
		A_{1}^{norm} X_{\mathcal V_1}^{(l)} W_1^{(l)} \\
		\vdots \\
		A_{K}^{norm} X_{\mathcal V_K}^{(l)} W_K^{(l)}
	\end{bmatrix})
	\label{eq.disttrain}
\end{equation}
where $X_{\mathcal V_k}^{(l)}$ represents the features of all nodes in $\mathcal V_k$ in the $l$-th layer. 
The nice property of the diagonal matrix $\tilde A$ allows us to perform local training on $K$ devices without the need of communicating node features among various devices.

\textbf{Graph Partitioning Objective.} So far, we have demonstrated that replacing $A$ with $\tilde A$ greatly improves training efficiency and scalability. The remaining problem is to find an \emph{optimal} graph partitioning strategy that outputs $\tilde A$. It is natural to conclude that the objective is: 
\begin{equation}
	\min_\mathcal{P} \sum_{i,j} (A_{ij}- \tilde A_{ij})
	\label{part}
\end{equation}
Thus, we aim at minimizing the number of non-zero elements for the error matrix $E$. In other words, the objective is to \emph{minimize the number of edges of incident nodes} that belong to different subsets. In fact, this is identical to the goal of various existing graph partitioning methods, making these approaches good candidates to use with our framework. We advocate using METIS \cite{metis} due to its efficiency in handling large-scale graphs. However, traditional graph partitioning algorithms are not intended for modern GNNs and the learning component of the problem is overlooked. Consequently, we present a modified version of METIS that is better suited to our problem.

\textbf{Weighted Graph Construction}. We build a weighted graph $\mathcal G^w$ from the input graph $\mathcal G$. The \emph{weight} of an edge $e_{uv}$ is defined based on the degree of its two incident nodes: 
\begin{equation}
 \begin{split}
	& weight(e_{uv}) = d_{max} + 1 - deg(u) - deg(v) \\
	& d_{max} = max\{deg(u)+deg(v), \forall e_{uv} \in \mathcal E \}
\end{split}
\label{eq.weighted_graph}
\end{equation}

We use $A^w$ to denote the adjacency matrix of the weighted graph $\mathcal G^w$, where element $a_{ij}^w$ denotes the edge weight $weight(e_{ij})$; $a_{ij}^w$ is 0 if there is no edge connecting node $i$ and $j$. Consequently, instead of minimizing the number of non-zero elements in $E$ (a binary matrix), we aim at minimizing the sum of elements in $E^w = A^w-\tilde A^w$. 

The key intuition of our design lies in the neighborhood aggregation scheme of GNNs. Consider two nodes $u$ and $v$, where $u$ is a hub node connected to many nodes, while $v$ has only one neighbor. As GNNs propagate by aggregating the neighborhood information of nodes, removing the only edge of node $v$ may possibly lead to wrong predictions. On the other hand, pruning an edge of $u$ is more acceptable since there are many neighbors contributing to its prediction. Consider the graph in Figure \ref{fig.framework} as an example, which provides an illustration of \sg for a two-device setup. Cutting the edges $e_1\cup e_2$ and $e_3\cup e_4$ are both feasible solutions for METIS. However, considering the fact that nodes connected to $e_1$ and $e_2$ have less topology information, the modified METIS we propose will preserve them and cut edges $e_3\cup e_4$ instead; this can lead to a better performance in GNNs.

As can be concluded from this small example, edges connected to small-degree nodes are critical to our problem and should be preserved within $\tilde A^w$. Conversely, edges connected to high-degree nodes may be intentionally ignored and placed in $E^w$. This explains our weights definition strategy. 
% Consequently, we incorporate the above observation into our partition objective and extend METIS on the pre-processed graph $G^w$.

\textbf{Subgraph Expansion}. After obtaining the partitions with our modified METIS, we propose to expand the subgraph based on available hardware resources. Although METIS only provides partitioning results where the node sets do not overlap, our proposed general formulation in Section \ref{sec.form} allows nodes to belong to multiple partitions. This brings great flexibility to our approach to adjust the node number for each device according to its memory budget. 

Suppose the available memory of device $k$ is larger than the actual requirement of training a GNN on subgraph $k$ (\ie, $H(\mathcal{SG}_k,W_k) < B_{MEM}^k$), then we may choose to expand the original subgraph $\mathcal{SG}_i$ to its one-hop neighbors. To be specific, we expand the node set $\mathcal{V}_k$ by adding the one-hop neighbors of nodes that do not belong to $\mathcal{V}_k$. As illustrated in Figure \ref{fig.framework} (a), we may expand the node set of the subgraph on device 0 (marked in light brown) to include node $n_{0}$ as well. While expanding the subgraph is likely to yield higher accuracy, training time and memory requirement will also increase. Therefore, we consider it as an optional step. 
% 
\subsection{Putting it all together}
To sum up, the \sg algorithm is detailed below.

\begin{algorithm}[htb]
   \caption{\sg}
   \label{alg.sgtrain}
   \hspace*{0.02in} {\bf Input:} 
   graph $\mathcal{G} = (\mathcal V,\mathcal E)$; node feature matrix $X$; available device number $K$; device memory budget $\{B_{MEM}^k\}_{k=1}^K$; total training epochs $T$.
\begin{algorithmic}[1]
   \STATE Construct $\mathcal G^w$ from $\mathcal G$ according to Equation \ref{eq.weighted_graph}
   \STATE Partition $\mathcal G^w$ into $K$ subgraphs $\{\mathcal{SG}_i\}_1^K$ 
   \STATE (Optional) Expand $\mathcal{SG}_i$ if $H(\mathcal{SG}_i,W_i) < B_{MEM}^i$
   \FOR{each device $k=\{1,2,\cdots,K\}$ in parallel}
   \STATE Initialize GNN model weight $W_k$
   \FOR{epoch $t=1,2,\cdots,T$}
   		\STATE $W_k^{t+1} = W_k^{t} - lr\bigtriangledown F_k(\mathcal{SG}_k; W_k^t)$ 
   	% 	\\ \COMMENT {Perform local model updates}
   		\ENDFOR
   \ENDFOR
   \STATE Calculate node predictions $Z_i = f(x_i;\mathbf{W}_i)$ according to Equation \ref{eq.formulation}
\end{algorithmic}
\end{algorithm}

\sg consists of two stages: (a) graph partitioning (lines 1-3) and (b) subgraph-level GNN training (lines 4-9). Before the training starts, \sg partitions the input graph and returns a set of subgraphs. Specifically, graph partitioning involves three steps: (1) construct a weighted graph $\mathcal G^w$ from $\mathcal G$ to account for the influence of node degrees in GNN learning (line 1). (2) Apply METIS to the weighted graph $\mathcal G^w$ to obtain partitioning results (line 2). (3) According to the memory budget, expand the subgraph to cover the one-hop neighbors for better performance (line 3). Then, we train $K$ local models in parallel and manage to reduce communication to zero through a few careful steps (lines 4-9). We demonstrate that subgraph-level training in a distributed fashion leads to reduced training time, smaller memory requirements and zero communication. 
% Figure \ref{fig.framework} provides an illustration of \sg for a two-device setup.

% As shown, \sg provides a general framework that targets local training in a resource-limited scenario, where mainstream GNN training methods are typically infeasible due to memory or communication costs.

%Note that contradictory to distributed learning approaches where communication is required in every round, we base our setting on an IoT scenario where communication during training time is not guaranteed. 

